A Secure Blockchain-Assisted Framework for Real-Time Maritime Environmental Compliance Monitoring

The maritime industry is governed by stringent environmental regulations, most notably the International Convention for the Prevention of Pollution from Ships (MARPOL). Ensuring compliance with these regulations is difficult due to low inspection rates and the risk of data fabrication. To address these issues, this paper proposes a secure blockchain-assisted framework for real-time maritime environmental compliance monitoring. By integrating IoT and shipboard sensors with blockchain technology, the framework ensures immutable and transparent record-keeping of environmental data. Smart contracts automate compliance verification and notify relevant authorities in case of non-compliance. A proof-of-concept case study on sulfur emissions demonstrates the framework's efficacy in enhancing MARPOL enforcement through real-time data integrity and regulatory adherence. The proposed system leverages the Polygon blockchain for scalability and efficiency, providing a robust solution for maritime environmental protection. The evaluation results demonstrate that the proposed blockchain-enhanced compliance monitoring system effectively and securely ensures real-time regulatory adherence with high scalability, efficiency, and cost-effectiveness, leveraging the robust capabilities of the Polygon blockchain.

==> Datasets.tex <==
\subsection{A List of GitHub Source Codes}
In our research, the datasets generated by Deepconfuse, error-minimizing, error-maximizing, and synthetic approaches were obtained from ~\cite{yu2021indiscriminate}. The datasets created by other approaches- autoregressive, OPS, SEP, EntF, REM, Hypocritical, and TensorClog were generated using the available code in their respective GitHub repositories. The links for GitHub repositories are provided in Table~\ref{tab:sourcecodes}.


\begin{table*}[h]
\scriptsize
%\small
    \centering
    \begin{tabular}{|p{3.5cm}|p{11cm}|}
    \hline
    Protection approach & Source code \\
    \hline
        NTGA & \url{https://github.com/lionelmessi6410/ntga?tab=readme-ov-file#unlearnable-datasets}\\
        \hline
        Autoregressive & \url{https://github.com/psandovalsegura/autoregressive-poisoning} \\
        \hline
        OPS & \url{https://github.com/cychomatica/One-Pixel-Shotcut}\\
        \hline
        SEP & \url{https://github.com/Sizhe-Chen/SEP}\\
        \hline
        EntF & \url{https://github.com/WenRuiUSTC/EntF}\\
        \hline
        REM & \url{https://github.com/fshp971/robust-unlearnable-examples}\\
        \hline
        Hypocritical & \url{https://github.com/TLMichael/Delusive-Adversary/tree/main} \\
        \hline
        TensorClog & \url{https://github.com/JC-S/TensorClog_Public}\\
        \hline
    \end{tabular}
    \caption{List of GitHub source codes.}
    \label{tab:sourcecodes}
\end{table*}

%In our research, the datasets generated by Deepconfuse, error-minimizing, error-maximizing, and synthetic approaches were obtained from ~\cite{yu2021indiscriminate}. The datasets created by other approaches- autoregressive, OPS, SEP, EntF, REM, Hypocritical, and TensorClog were generated using the available code in their respective GitHub repositories. The links for GitHub repositories are provided in Table~\ref{tab:sourcecodes}.

==> author_discussion.tex <==
\subsection{Guidelines}
Pixel manipulation is used on all data sets to increase the training data sets.

For the ImagaDataGenerator from Keras, the following were commonly used: zoom range (values = 0.3, 0.1, 0.4, 0.1, 0.4), rotation range (values = 7, 2, 10, 7, 7), and a horizontal flip.
Dilating is also used for all unlearnable CIFAR-10 datasets but not for unlearnable ImageNet dataset.

\textcolor{teal}{\sout{(Git) Based on what I noticed during the experiments, I suggest the following guideline.} \textcolor{red}{(Ks comment: You can include the limitation of the proposed methodology or experimental methods with potential solutions in the Discussion section. Moreover, people usually use the Discussion section to discuss some uncertain things or somethings you do not have answers yet. You may also include somethings you have done a little bit but incomplete work, where you may provide your insight about the work. You may further include some challenges you have encountered and will encounter with some of your thoughts or potential approaches to addressing them. Again. You need to emphasize on discussions with your thoughts, insights, etc.)} First, you start with data augmentation; I recommend using the OpenCV package. We noticed that pixel manipulation and dilating the poisoned images during the experiments are helpful. Then I would start using the ImageDataGenerator; this is again trial and error. However, we noticed that the following helpt increased the test accuracy for most data sets; a zoom range from 0.1-0.4, a rotation range from 2-10, but 7 was the most common one. And also include a horizontal flip. When you have the best combination of data augmentation, you start by experimenting with the number of epochs and learning rate. Best to do everything one by one and only keep the ones that increase the test accuracy. We used VGG16 and VGG19 as base models when working with the CIFAR-10 data set.}

\textcolor{blue}{\sout{(Thushari) According to my experience during the experiments, I can make the following suggestions.} \textcolor{red}{(KX's comment: See my comments in the previous paragraph.)} In order to make unlearnable data to learnable, increasing training dataset seems essential. You may try increasing the training set step by step using dilate, erode, pixel manipulation and gaussian blur techniques in OpenCV. Thresh binary and thresh binary inverse techniques also seems effective but make sure that the resulting images make sense before implementing. Keras ImageDatagenerator also provides useful attributes which make data more learnable. We suggest starting with horizontal flip, zoom range, and rotation range for that function. When it comes to the model, VGG16 or VGG19 are suitable for unlearnable CIFAR-10 dataset. We can also propose ResNet152 for ImageNet dataset based on our experiments. You can improve the model adding several FC layers and dropout layers until you the reach expected accuracy. We also experienced that changing learning rate has a considerable impact on increasing accuracy.}

\subsection{Discussions}

\textcolor{teal}{While training the poisoned images with NTGA, we also tried using ResNet 50. However, we did not try other ResNet architectures, so it might be that these give higher test accuracy.}
\textcolor{blue}{In this study, we used three unlearnable datasets with NTGA (MNIST,CIFAR-10,ImageNet) for our experiments. However, we only used CIFAR-10 dataset under all other data protection approaches. It would be more effective and balanced if we could conduct experiments for all three datasets under every attack not only NTGA. We also noticed that data augmentation techniques; thresh binary and thresh binary inverse do not provide meaningful images for unlearnable CIFAR-10 datasets. Hence, we avoided using those techniques for CIFAR-10, even though they had considerable impact on the test accuracy.  }

==> discussion_thoughts.tex <==
It is natural to think that augmentation policies may be a dead end against unlearnable attacks, as none of the existing strong data augmentation methods show significant effectiveness (Table 3). Adversarial training can also be viewed as a practical data augmentation policy, which presents an interesting perspective as it allows the model to choose its own policy in the form of `p-bounded perturbations adaptively. However, it poses a considerable challenge due to its use of large defensive perturbations, often resulting in reduced accuracy. This begs the question of whether new defense mechanisms can leverage unseen threat models that unlearnable attacks may be unable to account for.

==> relatedWork.tex <==
\textcolor{blue}{Adversarial examples are a critical challenge in machine learning, where models are deceived into making incorrect classifications. This deception occurs through the introduction of adversarial perturbations to source images, which are typically imperceptible to humans yet lead to erroneous outcomes \cite{goodfellow2014explaining}. A prominent technique in this field is white-box adversarial attacks \cite{DBLP:conf/iclr/MadryMSTV18}, which employ gradient descent on the defending model. The goal here is to add adversarial perturbations to an image in a way that maximizes its loss when analyzed by the model.}

\textcolor{blue}{To combat these threats, adversarial training has emerged as an effective method \cite{DBLP:conf/iclr/MadryMSTV18}. This approach involves incorporating adversarial examples into the training process of models, thereby enhancing their resilience to such attacks. The adversarial training algorithms focus on a min-max problem, aiming to minimize the loss function against the majority of adversarial examples, within a constraint often described as a perturbation budget, typically bounded in `p-norm. This field has seen a rapid evolution in recent years, marked by an intense competition between developing advanced adversarial attack strategies and creating robust defense mechanisms \cite{gao2022mora, yu2021lafeat}. This dynamic has significantly propelled research and innovation in machine learning security, emphasizing the importance of robust model development.}

\textcolor{blue}{Unlearnable example attacks represent a nuanced approach in the realm of data poisoning, where the objective is to hinder effective learning from these examples through carefully bounded perturbations. Distinct from classic data poisoning tactics, these methods typically involve adding subtle, almost imperceptible disturbances to all examples in a dataset \cite{DBLP:conf/iclr/FuHLST22, DBLP:conf/iclr/HuangME0021, tao2021better, yu2022availability, DBLP:journals/corr/abs-2206-03693}.}

\textcolor{blue}{One notable method is the Error-Minimizing (EM) poison \cite{DBLP:conf/iclr/HuangME0021}, which creates these minimal perturbations with a specific goal: to minimize the errors of training examples on a pretrained model. This approach, however, leads deep learning models to pick up on these 'shortcuts' rather than learning from the actual data, effectively making the examples hard to learn. Another strategy, Hypocritical perturbations (HYPO) \cite{tao2021better}, shares a similar concept but relies on a pretrained surrogate model for its implementation, diverging from the min-min optimization used in EM.}

\textcolor{blue}{Further, a Convolution-based Unlearnable Dataset (CUDA) generation technique that doesn't rely on specific models was proposed by Sadasivan \textit{et al.} \cite{sadasivan2023cuda}. CUDA uses class-specific convolutions with randomly generated filters, keyed privately, to encourage networks to learn filter-label relations instead of focusing on informative features for classifying clean data. However, these methods face challenges against adversarial training. To address this, the Robust Error-Minimizing (REM) technique \cite{DBLP:conf/iclr/FuHLST22} utilizes an adversarially-trained model to create more potent unlearnable examples. Similarly, INF \cite{wen2022adversarial} focuses on making samples from different classes share non-discriminatory features, thereby enhancing their resistance to adversarial training.}

\textcolor{blue}{Wu et al. \cite{wu2022one} demonstrated DNNs can be significantly impacted by perturbing just a single pixel in an image. Their method modifies one pixel in each training image in a specific way, causing the network to focus on this small change rather than learning semantic features of the image. Linear-separable Synthetic Perturbations (LSP) \cite{yu2022availability} also introduce a new perspective, showing that if the perturbations of unlearnable samples are aligned with their target labels, they become linearly separable. This insight led to the development of linearly separable perturbations, which have shown significant effectiveness. Further, Autoregressive poisoning (AR) \cite{DBLP:journals/corr/abs-2206-03693} proposes a universal perturbation approach applicable across various datasets and architectures. The AR method generates its perturbations through dataset-independent processes, adding another layer of complexity to the unlearnable examples landscape.}

\textcolor{blue}{Chen et al. \cite{chen2022self} propose the Self-Ensemble Protection (SEP) method, which uses intermediate model training checkpoints to create a self-ensemble for data protection. SEP effectively harnesses the diversity in the gradients of these checkpoints to generate protective perturbations. This approach allows for efficient ensemble performance by training only one deep neural network (DNN), making it a practical solution for large-scale data protection. To counteract the Perturbative Availability Poisons (PAPs), Liu et al. \cite{liu2023image} introduced Image Shortcut Squeezing (ISS) method, which uses imple image compression techniques. This method restores the accuracy of poisoned Deep Neural Network (DNN) models by applying specific compression operations like JPEG and grayscale transformation to eliminate both low and high-frequency perturbations introduced by PAPs.}



\textcolor{blue}{Moreover, data augmentation is a technique that enhances the variety of training data for machine learning models by applying a range of random transformations to images, such as rotation, flipping, and cropping \cite{krizhevsky2017imagenet}. These alterations help improve the model's ability to generalize to new data. Advanced techniques like TrivialAugment \cite{muller2021trivialaugment} and AutoAugment \cite{cubuk2019autoaugment} utilize automatic, search-based methods to identify a diverse set of augmentation policies, further enhancing the performance of deep neural networks (DNNs).}

\textcolor{blue}{An innovative approach in this domain is TorMentor \cite{nicolaou2022tormentor}, an image-augmentation framework that employs fractal-based data augmentation to bolster model generalization capabilities. Additionally, recent methods for creating unlearnable examples \cite{DBLP:conf/iclr/FuHLST22, DBLP:conf/iclr/HuangME0021, DBLP:journals/corr/abs-2206-03693, tao2021better} have shown impressive resilience against a wide array of data augmentation techniques. Contrary to the common assumption that these methods are ineffective against unlearnable examples, UEraser \cite{qin2023learning} introduces a novel strategy. It seeks out adversarial policies that maximize errors through augmentations, setting a new benchmark in defense performance against unlearnable example attacks.}

\textcolor{brown}{While Qin et al. \cite{qin2023learning} propose a defense mechanism that uses error-maximizing data augmentations to counteract unlearning effects in poisoned training data, our methodology revolves around constructing and deploying an attack on neural networks' generalization, exploring the experimental aspects of neural tangent kernels. Further, our paper contributes to understanding and exploiting the vulnerabilities in neural networks, providing insights into the limits of their generalization abilities. UEraser \cite{qin2023learning}, on the other hand, contributes a defense mechanism against data poisoning, using a combination of adversarial and data augmentation techniques to improve model resilience.}

\textcolor{blue}{In contrast to existing methodologies, our research uniquely explores the weaknesses in how neural networks generalize. We introduce a novel mechanism to attack these weaknesses, focusing on the theoretical exploration of neural tangent kernels. This approach involves the development and implementation of an attack strategy specifically targeting the generalization aspect of neural networks.}

==> table6.tex <==
%\begin{footnotesize}
\begin{table*}%[ht!]
%\footnotesize
\small
\begin{tabular}
{|>{\raggedright}P{1.8cm} |>{\raggedright}P{3.5cm}|>{\raggedright}P{5.1cm}|>{\raggedright}P{1.1cm}|>{\raggedright}P{1.1cm}|>{\raggedright\arraybackslash}P{0.8cm}|}
 \hline
 Protection approach & Nonlinear Transformations  &  Attributes for Keras ImageDataGenerator & Baseline model & Learning rate & \# of epochs \\
 \hline
 \hline
 NTGA & color channel manipulation (thrice) & otation range of 7, zoom range of 0.3, width and height shift range of 0.35, horizontal flip, shear range of 0.4 & VGG19 & 0.008 & 40 \\
 \hline
 Deepconfuse & dilate, erode, and color channel manipulation (twice) & rotation range of 7, width shift range of 0.3, horizontal flip, zoom range of 0.1 & VGG19 & 0.007 & 80 \\
 \hline
 Error-minimizing & dilate, erode, color channel manipulation (twice), and Gaussian blur &  rotation range of 7, height and width shift range of 0.3, horizontal flip,  zoom range of 0.1 & VGG16 & 0.006 & 80 \\
 \hline
 Error-maximizing & dilate, erode, and color channel manipulation (twice) & rotation range of 10,  shear range of 0.4, height and width shift range of 0.4, horizontal flip, zoom range of 0.4 &  VGG16 & 0.008 & 80  \\
 \hline
 Synthetic & dilate, erode, and color channel manipulation (twice) &rotation range of 7, width and height shift range of 0.3, shear range of 0.4, horizontal flip, zoom range of 0.4 & VGG19 & 0.007 & 40 \\
 \hline
 Autoregressive & dilate, erode, and color channel manipulation (twice) & rotation range of 7, horizontal flip, zoom range of 0.1 & VGG19 & 0.001 & 10
 \\
 \hline
  OPS &  dilate, erode, and color channel manipulation (twice) &  rotation range of 7, width and height shift range of 0.3, horizontal flip, zoom range of 0.1 &  VGG19 &  0.001  &  30 \\
 \hline
  SEP &  color channel manipulation (twice) &  rotation range of 7, width and height shift range of 0.1, horizontal flip, zoom range of 0.1 &  VGG16 &  0.001  &  50 \\
 \hline
  EntF &  erode and color channel manipulation &  rotation range of 7, width and height shift range of 0.3, horizontal flip, zoom range of 0.1 &  VGG19 &  0.001  &  30 \\
 \hline
   REM &  erode and color channel manipulation (twice) &  rotation range of 7, width shift range of 0.15, and height shift range of 0.2, horizontal flip, zoom range of 0.1 &  VGG16 &  0.006  &  80 \\
 \hline
   Hypocritical &  dilate, erode and color channel manipulation &  rotation range of 7, width and height shift range of 0.3, horizontal flip, zoom range of 0.1 &  VGG19 &  0.001  &  30 \\
 \hline
  TensorClog &  dilate, erode and color channel manipulation &  rotation range of 7, width and height shift range of 0.3, horizontal flip, zoom range of 0.1 &  VGG19 &  0.001  &  30 \\
 \hline
 \end{tabular} 
\caption{Summary of transformations and model specifications used to make these unlearnable CIFAR-10 images learnable.}
 \label{t:6}
\end{table*}
%\end{footnotesize}

==> tables.tex <==
% -------------------------------------------------
\begin{table}[ht!]
\small
\centering
   \begin{subtable}[b]{0.48\textwidth}
    \begin{tabular}{|c c c|} 
    \hline
    Layer & Output shape & Activation function \\  
    \hline
    Input  & 28 x 28 x 1 &  \\ 
    \hline
    Convolutional   & 28 x 28 x 32 & ReLU \\
    \hline
    Max pool & 14 x 14 x 32  &  \\
    \hline
    Convolutional & 14 x 14 x 64 & ReLU  \\
    \hline
    Max pool & 7 x 7 x 64 &  \\ 
    \hline
    Flatten &  & \\
    \hline
    FC & 1024 & ReLU\\
    \hline
    Dropout (0.25) & 1024 & \\
    \hline
    FC & 10 & Softmax\\
    \hline
    \end{tabular}
    \caption{MNIST}
    \label{fig:modelmnist}
    \end{subtable}
    \begin{subtable}[b]{0.48\textwidth}
    \begin{tabular}{|c c c|} 
    \hline
    Layer & Output shape & Activation function \\  
    \hline
    Input  & 32 x 32 x 3 &   \\ 
    \hline
    2 x Convolutional   & 32 x 32 x 64 & ReLU \\
    \hline
    Max pool & 16 x 16 x 64  &  \\
    \hline
    2 x Convolutional & 16 x 16 x 128 & ReLu  \\
    \hline
    Max pool & 8 x 8 x 128 &  \\ 
    \hline
 4 x Convolutional & 8 x 8 x 256 & ReLU \\
    \hline
    Max pool & 4 x 4 x 256 & \\ 
    \hline
    4 x Convolutional & 4 x 4 x 512 & ReLU\\
    \hline
    Max pool & 2 x 2 x 512 &\\
    \hline
    4 x Convolutional & 2 x 2 x 512 & ReLU\\
    \hline
    Max pool & 1 x 1 x 512 & \\
    \hline
Flatten & 512 &\\
    \hline
    FC & 1024 & ReLU \\
    \hline
    Dropout (0.3) & 1024 & \\
    \hline
    FC & 512 & ReLU \\
    \hline
    Dropout (0.3) & 512 & \\
    \hline
    FC & 64 & ReLU\\
    \hline 
    FC & 10 & Softmax\\
    \hline
    \end{tabular}
    \caption{CIFAR-10}
    \label{fig:modelcifar}
    \end{subtable}
    \begin{subtable}[b]{0.48\textwidth}
        \begin{tabular}{| c c c| }
     \hline
     Layer  & Output shape & Activation function \\
     \hline
     Input & 224 x 224 x 3 & \\
     \hline
     7 x 7, 64, / 2 & 112 x 112 x 64 & ReLU\\  
     \hline
     3 x 3 max pool, / 2 & 56 x 56 x 64 & \\ 
     \hline $\begin{bmatrix} 1 \times 1 ,64\\ 3 \times 3 ,64\\ 1 \times 1 ,256 \end{bmatrix}$ x 3 & 56 x 56 x 64 & ReLU\\[0.5cm]
     \hline
     $\begin{bmatrix} 1 \times 1 ,128\\ 3 \times 3 ,128\\ 1 \times 1 ,512
     \end{bmatrix}$ x 8 & 28 x 28 x 128 & ReLU\\[0.5cm]
     \hline
     $\begin{bmatrix} 1 \times 1 ,256\\ 3 \times 3 ,256\\ 1 \times 1 ,1024
     \end{bmatrix}$ x 36 & 14 x 14 x 256 & ReLU \\[0.5cm]
     \hline
     $\begin{bmatrix} 1 \times 1 ,512\\ 3 \times 3 ,512\\ 1 \times 1 ,2048
     \end{bmatrix}$ x 3 & 7 x 7 x 512 & ReLU \\[0.5cm]
     \hline
     $\begin{bmatrix} 1 \times 1 ,512\\ 3 \times 3 ,512\\ 1 \times 1 ,2048
     \end{bmatrix} $ x 3 & 1 x 1 x 512 & ReLU  \\[0.5cm] \hline
     Average pool & 1 x 1 x 512 & Softmax\\ \hline
     Flatten & 512 &\\ \hline
     FC & 1024 & ReLU \\ \hline
     Dropout (0.3) & 1024 &\\ \hline
     FC & 512 & ReLU\\ \hline
     FC & 256 & ReLU \\ \hline
     FC & 128 & ReLU \\ \hline
     FC & 64 & ReLU \\ \hline
     FC & 2 & Softmax \\ \hline
     \end{tabular}
    \caption{ImageNet}
     \label{fig:ImageNet model}
    \end{subtable}
    \caption{The model architecture used for training each unlearnable  dataset crafted by NTGA.}
\end{table}
